On expansions of non-abelian free groups by cosets of a finite index subgroup

Let $F$ be a finitely generated non-abelian free group and $Q$ a finite quotient. Denote by $L_Q$ the language obtained by adding unary predicates $P_q$, $q\in Q$ to the language of groups. Using a slight generalization of some of the techniques involved in Zlil Sela's solution to Tarski\'s problem on the elementary theory of non-abelian free groups, we provide a few basic results on the validity of first order entences in the $L_Q$-expansion of $F$ in which every $P_q$ is interpreted as the preimage of $q$ in $F$. In particular we prove an analogous result to Sela's generalization of Merzlyakov's theorem on $\forall\exists$-sentences and show that the positive theory depends only on $Q$ and neither on the rank of $F$ nor the particular quotient map.

==> abstract/deutsches_abstract <==
	Let $\F$ be a finitely generated non-abelian free group and $Q$ a finite quotient. Denote by $\LQ$ the language obtained by adding unary predicates $\{P_{q}\}_{q\in Q}$ to the language of groups.
	
	By generalizing some of the techniques involved in Zlil Sela's solution to Tarski's question on the elementary theory of non-abelian free groups, we provide a few basic results on the validity of first order sentences in the $\LQ$-expansion of $\F$ in which every $P_{q}$ is interpreted as the preimage of $q$ in $\F$.
	
	In particular, we prove an analogous result to Sela's generalization of Merzlyakov's theorem for $\forall\exists$-sentence and show that the positive theory of such a structure depends only on $Q$ and not on the rank of $\F$ nor the particular quotient map.


Wir betrachten die Struktur der ersten Stufe erhalten indem man zu der Gruppenstruktur einer nicht abelischen freien Gruppe ein Predikat für jede der Fasern eines surjektiven Homomorphismus von der freien Gruppe in eine endliche Gruppe hinzufügt. Wir dass die positive Theorie der so enstandenen Struktur nür von der endlichen Gruppe abhängig ist. 


